ViMo: Generating Motions from Casual Videos

Although humans have the innate ability to imagine multiple possible actions from videos, it remains an extraordinary challenge for computers due to the intricate camera movements and montages. Most existing motion generation methods predominantly rely on manually collected motion datasets, usually tediously sourced from motion capture (Mocap) systems or Multi-View cameras, unavoidably resulting in a limited size that severely undermines their generalizability. Inspired by recent advance of diffusion models, we probe a simple and effective way to capture motions from videos and propose a novel Video-to-Motion-Generation framework (ViMo) which could leverage the immense trove of untapped video content to produce abundant and diverse 3D human motions. Distinct from prior work, our videos could be more causal, including complicated camera movements and occlusions. Striking experimental results demonstrate the proposed model could generate natural motions even for videos where rapid movements, varying perspectives, or frequent occlusions might exist. We also show this work could enable three important downstream applications, such as generating dancing motions according to arbitrary music and source video style. Extensive experimental results prove that our model offers an effective and scalable way to generate diversity and realistic motions. Code and demos will be public soon.

==> section/0_Abstract.tex <==
\begin{abstract}
Although humans have the innate ability to imagine multiple possible actions from videos, it remains an extraordinary challenge for computers due to the intricate camera movements and montages. Most existing motion generation methods predominantly rely on manually collected motion datasets, usually tediously sourced from motion capture (Mocap) systems or Multi-View cameras, unavoidably resulting in a limited size that severely undermines their generalizability. Inspired by recent advance of diffusion models, we probe a simple and effective way to capture motions from videos and propose a novel Video-to-Motion-Generation framework (ViMo) which could leverage the immense trove of untapped video content to produce abundant and diverse 3D human motions. Distinct from prior work, our videos could be more causal, including complicated camera movements and occlusions. Striking experimental results demonstrate the proposed model could generate natural motions even for videos where rapid movements, varying perspectives, or frequent occlusions might exist. We also show this work could enable three important downstream applications, such as generating dancing motions according to arbitrary music and source video style. Extensive experimental results prove that our model offers an effective and scalable way to generate diversity and realistic motions. Code and demos will be public soon.
\end{abstract}

%Additionally, a novel ``Rhythm" metric is designed to measure the semantic divergence of 2D content and 3D motions for the first time. 

==> section/XXX_old_1_Introduction.tex <==
\section{Introduction}

% (1) mocap expensive and time actor costly, so we need motion generation 
Realistic 3D human motions play an important role as the `soul' of virtual characters since they can make them feel alive – it enables the static character to jump, fight and dance~\cite{aberman2020skeleton}. With the rapid proliferation of portable devices and the metaverse, the demands on virtual character creation are rising at an explosive rate. In the traditional animation and film industry, the motions are created manually in a tedious way either by expensive motion capture systems~\cite{menolotto2020motion} or by professional animators, therefore usually resulting in a very time-consuming and laborious process. Motivated by this problem, data-driven motion generation methods~\cite{tseng2023edge,raab2022modi,tevet2022human,alexanderson2023listen,huang2023diffusion,zhang2022motiondiffuse} have been widely studied recently since they are super efficient and economical~\cite{zhang2023magicavatar}. 


%(2) Existing motion Generations are very limited on the generation domain-- so we need video as input
Although promising progress in motion generations has been achieved, the diversity and flexibility of the synthesised motions are still far behind the expectations of the users in practical applications. Most existing motion generation approaches adopt the diffusion-based, VAE or GAN-based framework and take condition signals which are input parameters or data types that guide the motion generation process, such as Gaussian noise~\cite{yan2019convolutional,raab2022modi}, text~\cite{tevet2022motionclip,tevet2022human,zhang2022motiondiffuse}, audio~\cite{liu2022audio,alexanderson2023listen}, music~\cite{aristidou2021rhythm,sun2020deepdance,li2022danceformer} or scene contexts~\cite{wang2022humanise,huang2023diffusion}. The effectiveness of these models is contingent upon the availability of matched accurate examples (ground-truth pairs) of both the input conditions (like audio or text) and the corresponding motions. Consequently, this way narrows the synthesised motions only to specific domains and finite categories provided in the training dataset. For example, the state-of-the-artwork EDGE~\cite{tseng2023edge} generated dancing movements are all limited to the 10 categories of street dancing provided in the training dataset AIST++~\cite{li2021ai}. The existing action-conditioned motion generations~\cite{degardin2022generative,maheshwari2022mugl, petrovich2021action,guo2020action2motion} are only able to generate motions in the same label of the input in the training dataset as well. 

%(3) Video is a large resource, we use video for motion 
The motion datasets hamper these generation methods from scaling up. This is because they are typically captured using professional Mocap Systems or Multi-View cameras which are time-consuming and costly. 
In contrast, video resources are incredibly extensive and widely available, offering a broader range of diverse and interesting human actions. 
However, this topic remains very under-exploited due to the significant complexity and variability of video content. 
There are some existing approaches~\cite{zhu2023motionbert,yuan2022glamr,ye2023decoupling,pavlakos2022human,pavllo20193d,cai2023smpler} explored to leverage the 3D pose estimation methods to reconstruct the 3D human motions precisely from video resources, therefore generating more diverse types of motions. For example, The state-of-the-artwork MotionBERT~\cite{zhu2023motionbert} can estimate high-fidelity 3D joint positions and perform natural human movements similar to the videos. 
However, their models are mostly only tested on videos with specific conditions --the camera position could be known accurately. When the videos include complex camera movements or montage editing techniques (Figure~\ref{fig:teaser}), their performance could degrade drastically and fall into collapse. However, most online videos that we denote as \textbf{Casual videos} usually unavoidably contain complex occlusions and camera movements, which are out of their assumption. 

Reconstructing 3D motions from these casual videos will be incredibly complicated, as estimating the complex camera angles and locations is overly intricate and sometimes not feasible.
Without accurate camera positions, the regression loss employed in the aforementioned methods will become completely dysfunctional and frame-wise poses are hard to string together as a smooth motion. Therefore, learning 3D motions from casual videos is a desirable goal but remains a formidable challenge due to the intricate camera issues. 

% as these 2D and 3D joint coordinates and trajectories would be utterly incomparable. 
% (5) So we propose a new pipeline and new task. 
In contrast, humans can easily comprehend 3D actions from casual videos. To capture the essence of actions in videos, the 3D motions just need to be similar in poses and rhythms rather than the high precision of joint locations. Inspired by that, we pose a new video-to-motion generation question -- \textit{could the computer generate multiple possible 3D motions of the new types according to the actions provided in the casual videos which have very similar pose shapes and rhythms? } % Illustratively, the 2D pose in each frame should look like a projection of the 3D skeleton, with both the trajectory transitions of the joints, including turns and stops, and their speeds being broadly similar.

%incorporates a newly devised \textbf{Rhythm Metric}, which assesses the consistency between the generated 3D motion and the source video. 
%Although the visualization results are significant, we are still curious about how to quantitatively measure the consistency between the 2D pose sequences and 3D motion when the camera changes. % The conditional signal and outputs are time sequences therefore the spatial-temporal information will be learned inherently in the diffusion process. The next challenge is, how to evaluate the rhythm similarity between a casual video and 3D motion?

% (7) what motion we want, similar to video (***)
%As claimed in literature~\cite{zhu2023human}, designing consistency metrics for conditional-based motion generation tasks is a crucial yet challenging problem. In this work, we explore designing an appropriate metric to measure the rhythm similarity between the 2D pose sequences and 3D motion. 
%We comprehensively investigate the relationship between 3D motion and their projected 2D pose sequences. Instead of absolute joint positions, we record the relative distance between symmetric joints (e.g. hand, feet) both in 2D and 3D situations and discover that most of these signals show similar frequency even under camera changes if they are from the same action. Although camera movements will introduce extra changes in the waveform of signals, it is neglectable compared with the dominant action signals. Therefore, we design a novel Rhythm metric by leveraging DCT (Discrete Cosine Transform) to broadly estimate the similarity between their turns, stops, and speeds. % We demonstrate that this loss could supervise the turns, stops and speed similarity during the 2D to 3D generation process, thus producing a sequence of 3D motions that could exhibit highly similar rhythm, but not identical joint locations to the video.

% (8) %Two applications to demonstrate the value and experiment results
To achieve this goal, we propose a novel video-to-motion generation model by taking videos as conditions to generate various motions and showcase its great potential in enabling three important downstream applications. Specifically, we introduce a diffusion-based framework which takes the 2D poses from multiple different views as the input data to generate 3D motions. With this design, our model can create a sequence of 3D motion without explicitly estimating the camera positions. 
We conducted extensive experiments to validate the effectiveness of our approach. The results reveal that this simple approach could effectively generate unlimited complex and realistic 3D motions which are contextually consistent with the input casual videos even when they contain complex camera movements and occlusions. Notably, we show that our work could enable three interesting downstream applications. (1) Firstly, it could be an efficient way to produce large-scale motion datasets. We collected a large-scale Chinese classic dancing dataset and built up a 3D dancing motion dataset that included 750 motions. This new dataset could be used to facilitate data-driven tasks such as music-to-dancing generation, motion recognition and prediction. (2) Secondly, our model could power up few-shot stylization in the dancing generation. Specifically, we could leverage the music-to-motion generation pipeline to generate a specific style of dance according to the pose style offered by a few video examples. (3) Thirdly, we could form a new video-guided motion completion and editing task which could fill in the missing part of the motion by the similar content defined by any source videos. 

% (9) Our contribution list 
In summary, we contribute in the following aspects to encourage future research towards this goal:
(1) We propose a novel video-to-motion-generation model to leverage the abundant resources of the actions in videos to enhance the diversity and realism of 3D motion generation. By posing this new question, we reveal that the diversity and flexibility of motion generation could be greatly extended by a simple but effective approach. 
%(2) We first introduce a Rhythm metric to measure the similarity of the 2D poses in videos and 3D motions. Importantly, the consistency of the video conditions and generated motions could be quantitatively measured under varying projections. %For the first time, the rhythm of 2D and 3D actions can be quantitatively measured under varying projection angles.
(2) A dancing specified 3D motion dataset is constructed with the proposed ViMo model, which contains 52 Chinese classic dancing videos together with 750 generated 3D dancing motions. This demontrate the effectiveness and advantages of video-to-motion-generation strategy. We hope suck kind of video-to-motion dataset could facilitate a lot of motion-related tasks.  
% such as generation, prediction and recognition. 
% 
(3) We demonstrate that the proposed method could be impressively activated in three real-life applications which illustrate its astonishing ability to generate realistic and aesthetical human motions. 


